Frustratingly Easy Natural Question Answering

Existing literature on Question Answering (QA) mostly focuses on algorithmic novelty, data augmentation, or increasingly large pre-trained language models like XLNet and RoBERTa. Additionally, a lot of systems on the QA leaderboards do not have associated research documentation in order to successfully replicate their experiments. In this paper, we outline these algorithmic components such as Attention-over-Attention, coupled with data augmentation and ensembling strategies that have shown to yield state-of-the-art results on benchmark datasets like SQuAD, even achieving super-human performance. Contrary to these prior results, when we evaluate on the recently proposed Natural Questions benchmark dataset, we find that an incredibly simple approach of transfer learning from BERT outperforms the previous state-of-the-art system trained on 4 million more examples than ours by 1.9 F1 points. Adding ensembling strategies further improves that number by 2.3 F1 points.

==> ensembling.tex <==
\section{Ensembling}
\label{sec:ensemble}
%\rishav{How about replacing the first sentence with this one to tie into the previous section and provide a bit more context: In addition to optimizing for single model performance, we investigate a number of strategies for ensembling models as is common for top ranking leaderboard submissions in MRC\footnote{The top ranking submissions for SQuAD 2.0, TriviaQA, and HotpotQA are all ensemble models as of this paper's writing.}}
%\anthony{Sounds good - added}
%We investigate a number of strategies for ensembling models.  
In addition to optimizing for single model performance, in this section we outline a number of strategies that we investigated for ensembling models as is common for top ranking leaderboard submissions in MRC\footnote{The top ranking submissions for SQuAD 2.0, TriviaQA, and HotpotQA are all ensemble models as of this paper's writing.}.
In order to formally compare approaches we partition the NQ dev set into ``dev-train'' and ``dev-test'' by taking the first three dev files for the ``train'' set and using the last two for the ``test'' set (the original dev set for NQ is partitioned into 5 files for distribution).  This yields ``train'' and ``test'' sets of 4,653 and 3,177 examples (query-article pairs)
%\rishav{Should we use ``queries'' or ``query-article pairs'' instead of ``examples'' since it seems unclear if we mean before or after splitting into multiple spans?} 
respectively.  For each strategy considered we search for the best k-model ensemble over the ``train'' set and then evaluate on the ``test'' set.  For these experiments we use $k=4$ as this is the number of models that we can decode in the 24 hours on a Nvidia\textsuperscript{\textregistered} Tesla\textsuperscript{\textregistered} P100 GPU, which is the limit for the NQ leaderboard.  We begin by outlining our core strategy that underlies the approaches we have investigated.  Using this core strategy we investigate a baseline approach of ensembling multiple versions of the same model trained with different seeds in addition to a number of search, normalization, and aggregation strategies and the impact they have on F1 performance.
% \rishav{The subsections under this ``Ensembling'' section seem a little disjointed; it might be helpful to split the last two sentences of the above paragraph and elaborate a little with some structure. It sounds like we describe 2 aspects of ensembling decisions: (1) given a set of models and the corresponding top 20 predicted spans for each model, how to compute a combined prediction score per predicted span (2) given a set of candidate models (of size $>$ 5), how to choose the optimal subset of size 5. Plus there are two side notes: (1) talk about how prediction spans need to be combined both across models as well as within models (2) score normalization}

\subsection{Core Strategy}
% Core underlying strategy
For each example processed by the $k$ systems being ensembled, our system assigns a score to each long and short span\footnote{Note that our system currently only predicts single short spans rather than sets, so we currently score each short span independently.} according to the normalization and aggregation strategies (see below).  We use the top-20 candidate long and short answers for each system and example as we have empirically found this to be beneficial to considering fewer candidates (e.g. 5 or 10).  To combine systems we take the arithmetic mean\footnote{We have experimented with other approaches such as median, geometric mean, and harmonic; however these are omitted here as they resulted in much lower scores than arithmetic mean.} of the scores for each long and short span predicted by at least one system.  For spans which are only predicted by some systems a score of zero is assigned (for the systems which do not predict the span) to penalize spans which are only predicted by some systems. The predicted long span is then the span with the greatest arithmetic mean.  Similarly for short answers the predicted span is the one with the greatest arithmetic mean, with the exception that it may not be contained within a null long span \rishav{we may have to either explain why long spans can be null or exclude this detail as it seems minor?  Or, @Avi, is it a major contributor to performance?}. 

\subsection{Seed Ensembles}
We first examine the baseline approach of ensembling $k$ versions of the same model trained with the same hyperparameters, only varying the seed between models.  We select the model with the highest sum of short and long answer F1 scores on dev.  These models are then ensembled using the core strategy.  


% Mention snooping of selecting based on full dev performance and how even with this it is worse.

\subsection{Search Strategies}
\rishav{Maybe as intro we need something like: In addition to exploring ensembles consisting of the best performing model configuration trained with multiple starting seeds, we employ a search over models trained with the diverse set of training strategies and architectures outlined in the previous sections (even those those strategies do not yield the single best performing model configurations).}
We consider a baseline strategy which we refer to as simple greedy and two main strategies when searching for ensembles: exhaustive and greedy.  In exhaustive search we consider all possible ensembles, whereas in greedy search we build the ensemble one model at a time by looking for which model we can add to an $i$ model ensemble to make the best $i+1$ model ensemble.


% \subsubsection{Simple Greedy}
% For the simple greedy approach we take our top-k models for short answer and long answer and create two different ensembles by utilizing our core strategy for each.

\subsubsection{Exhaustive Search}
We first consider the exhaustive search approach where we consider each of the ${n \choose k}$ ensembles of k candidates from our group of n models.
We then use our core strategy for each ensemble to obtain short and long answer F1 scores for each ensemble.
After searching all possible ensembles we return two ensembles: (i) the ensemble with the highest long answer F1 score and (ii) the ensemble with the highest short answer F1 score.

% % Core underlying strategy
% For each example processed by the $k$ systems being ensembled, our system assigns a score to each long and short span\footnote{Note that our system currently only predicts single short spans rather than sets, so we currently score each short span independently.} according to the normalization and aggregation strategies (see below).  To combine systems we take the arithmetic mean\footnote{We have experimented with other approaches such as median, geometric mean, and harmonic; however these are omitted here as they resulted in much worse scores than arithmetic mean.} of the scores for each long and short span predicted by at least one system.  For spans which are only predicted by some systems a score of zero is assigned (for the systems which do not predict the span) to penalize spans which are only predicted by some systems. The predicted long span is then the span with the greatest arithmetic mean.  Similarly for short answers the predicted span is the one with the greatest arithmetic mean, with the exception that it may not be contained with in a null long span. 

% After searching all possible ensembles we return two ensembles: (i) the ensemble with the highest long answer F1 score and (ii) the ensemble with the highest short answer F1 score.

\subsubsection{Greedy Search}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Full version
% We then consider the greedy approach.  In order to more precisely control the tradeoff between optimizing for short and long answers we add an additional parameter $0 \leq k_{S} \leq k$ to specify the number of models which should be used to optimize short answer performance (i.e. $k = k_{S}$ indicates to exclusively optimize for short answers).  This induces another parameter $k_{L} = k - k_{S}$, the number of models which are used to optimize for long answer performance.  We refer to these ensembles that will be created for short and long answers as $S$ and $L$ respectively.  

% We construct S by greedily building $1, 2, ..., k_{S}$ model ensembles optimizing for short answer F1 using our core strategy.  In case adding some of the models decreased our short answer performance, we take the first $i \leq k_{S}$ models of $S$ which give the highest short answer F1.  Similarly we construct $L$ by greedily building a $k_{L}$ model ensemble optimizing for long answer F1.

% Since we are already decoding all of the models in $L$, we check to see if adding any subset of these models to $S$ improves short answer performance.  More formally we create $S^{\prime} = S \cup \argmax_{x \in \mathcal{P}(L)} F1_{S}(S \cup x)$ where $F1_{S}(X)$ is the short answer F1 for the ensemble created with the models in $X$.  We do the same for optimizing long answer performance, creating $L^{\prime} = L \cup \argmax_{x \in \mathcal{P}(S)} F1_{L}(L \cup x)$. 

% Finally, we join the predictions for short and long answers together by taking the short answer and long answer predictions from $S^{\prime}$ and $L^{\prime}$ respectively.  If for an example a null long answer is predicted, we also predict a null short answer regardless of what $S^{\prime}$ predicted as there are no short answers for examples which do not have a long answer in NQ \cite{Kwiatkowski2019NaturalQA}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Version with optimizing greedily just for SA or LA 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We then consider the greedy approach, optimizing for either short or long answer performance.  We refer to the ensembles created in this way as $S$ and $L$ respectively.

We construct $S$ by greedily building $1, 2, ..., k_{S}$ model ensembles optimizing for short answer F1 using our core strategy.  In case adding some of the models decreased our short answer performance, we take the first $i \leq k_{S}$ models of $S$ which give the highest short answer F1.  The same is done for $L$ when optimizing for long answers.
%Similarly we construct $L$ by greedily building a $k_{L}$ model ensemble optimizing for long answer F1.

%Since we are already decoding all of the models in $L$, we check to see if adding any subset of these models to $S$ improves short answer performance.  More formally we create $S^{\prime} = S \cup \argmax_{x \in \mathcal{P}(L)} F1_{S}(S \cup x)$ where $F1_{S}(X)$ is the short answer F1 for the ensemble created with the models in $X$.  We do the same for optimizing long answer performance, creating $L^{\prime} = L \cup \argmax_{x \in \mathcal{P}(S)} F1_{L}(L \cup x)$. 

To build the long answer ensemble (when optimizing for short answer performance), we check to see which subset of $S$ results in the best long answer performance.  More formally we create $L^{\prime} = \argmax_{x \in \mathcal{P}(L)} F1_{L}(x)$ where $F1_{L}(X)$ is the long answer F1 for the ensemble created with the models in $X$.  A correcsponding approach is used to create $L^{\prime}$ when optimizing for long answers.

Finally, we join the predictions for short and long answers together by taking the short answer and long answer predictions from our short and long answer model sets respectively.  If for an example a null long answer is predicted, we also predict a null short answer regardless of what $S^{\prime}$ predicted as there are no short answers for examples which do not have a long answer in NQ \cite{Kwiatkowski2019NaturalQA}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Normalization Strategies}
We investigate two primary methods for normalizing the scores predicted for a span: not normalizing and logistic regression\footnote{We also investigated normalizing by dividing the scores for a span by the sum of all scores for the span, however we omit these results for brevity as they did not produce interesting results.}.

\subsubsection{None}
As a baseline we run experiments where the scores for a span are used as-is.

\subsubsection{Logistic Regression}
We also experiment with normalization using logistic regression where the scores from the top prediction for the ``dev-train'' examples is used to predict whether the example is correctly answered\footnote{In our experiments using the top example performed equally well to using the top 20 predictions per example to train on.}.  To ensure an appropriate regularization strength is used, we use the scikit-learn \cite{scikit-learn} implementation of logistic regression with stratified 5-fold cross-validation to select the L2 regularization strength.

We also experimented with using other features such as the query length and normalizing the score with the mean and standard deviation of scores for that example, however this did not improve performance so they were omitted.  The nonnecessity of these additional features was confirmed both by feature selection and by comparing the F1 scores of the rescored predictions using a model trained with and without these features.

\subsection{Aggregation Strategies} % Add more to this section in general?
We consider a number of aggregation strategies to produce a single span for each span predicted by a system for an example.  These include the baseline approaches of max and sum as well as the exponentially decaying sum, (reciprocal) linearly decaying sum, and noisy or methods influenced by IR.  Note that all of these approaches operate on a vector $P$ of scores on which one of the above normalization strategies has been applied.

\subsubsection{Max}
We take the greatest score produced by a system for a span, or more formally for a vector $P$, $score = \max_{i=1}^{|P|} P_{i}$.

% Anthony: Skip
% \subsubsection{Sum} 
% For the sum method we take the sum of the scores produced by a system for a span, or more formally $score = \sum_{i=1}^{|P|} P_{i}$.

% Thoughts on whether this is worth including?  I didn't do the testing portion of this due to low train F1, will do testing if adding this to paper

\subsubsection{Exponential Sum}
We reverse sort $P$ and take $score = \sum_{i=1}^{|P|} P_{i} * \beta^{i - 1}$ for some constant $\beta$ (we use $\beta = 0.5)$.

\subsubsection{Linear Sum} % More accurate  name??
We reverse sort $P$ and take $score = \sum_{i=1}^{|P|} P_{i} * \frac{1}{i}$.

\subsubsection{Noisy Or}
We take $score = 1 - \prod_{i=1}^{|P|} (1 - P_{i})$.

% \subsection{Experiments}
% % Table showcasing experimental results on "train/test" split
% We examine two types of ensembling experiments: (i) ensembling the same model trained with different seeds and (ii) ensembling different models.  Ensembling different the same model trained on different seeds attempts to smooth the variance to produce a stronger result.  On the other hand ensembling different models attempts to find models that may not be the strongest individually but harmonize well to produce strong results.

% \subsubsection{Seed experiments}
% % Showing relative ineffectiveness of ensembling the same model with diff seeds
% In table \ref{tab:exp:seed} we find that there is a benefit to ensembling multiple versions of the same model trained with different seeds\footnote{Note that there is some data snooping ocuring here as models are selected based on full dev performance (which is a superset of ``dev-test'').}.

% \begin{table}[]
% \small
% \begin{tabular}{lll}
% \# Models  & SA F1 Eval & LA F1 Eval   \\
% 1  & 0.5614 & 0.6710  \\
% 4  & \textbf{0.5873} & \textbf{0.6961}  
% \end{tabular}
% \caption{Ensembling the same model trained with different seeds.  We find that training multiple versions of a model with different seeds and ensembling them increases performance.}
% \label{tab:exp:seed}
% \end{table}

% \subsubsection{Main experiments}
% % Table of experiments
% % Experiments that I can include:
% % Basic Greedy: 5
% % Basic Exhaustive: 2
% % Basic Greedy on candidates from Basic Exhaustive: 5 (probably just mention single summary sentence for these to save space)
% % Take top-k performing LA or SA on dev (snooping): 2
% % Greedy Sum: 5

% % Normalized:
% % Greedy Linearly Decaying Sum: 5
% % Greedy Exponentially Decaying Sum: 5
% % Greedy Noisy Or: 5

% % Follow up expts: 3

% % Notes:
% % - Almost all of the normalized expts use logistic regression that is snooping.  Ran 2 experiments with one that doesn't to confirm no impact of snooping
% % - Ran some informal expts (on candidates submitted to leaderboard last time) which showed that the aggregation expts needed normalization too.  Thinking I just mention that results for these are ommitted for brevity since they do not show anything interesting (other than that collectively they are poor results)
% % Maybe after basic expts just show optimizing for LA since that generalizes best
% % Columns: [Row, Search Strategy, Normalization Strategy, Aggregation Strategy, Num models searched, Num Models, Num SA models, Num LA models, SA F1 Search, LA F1 Search, F1 F1 Eval, LA F1 Eval]

% % Table \anthony{TODO: ref} shows several experiments with different search, normalization, and aggregation strategies.  We also investigated the IR aggregation approaches without normalization, however we omit these results here for brevity as they did not perform nearly as well as when normalization was applied.

% % - Greedy vs Exhaustive vs Simple Greedy [Search Strategy, Num models searched, Num SA models, Num LA models, SA F1 Search, LA F1 Search, F1 F1 Eval, LA F1 Eval]
% %     - Conclusion: Use greedy and all optimize for LA since they generalize better
% \begin{table*}[]
% \small
% \begin{tabular}{llllllll}
%  Search Strategy & \# Models Searched & \# SA Models & \# LA Models  & SA F1 Search & LA F1 Search & SA F1 Eval & LA F1 Eval   \\
%  Simple Greedy & 4 & 0 & 4 & N/A & N/A & 0.5925 & 0.6902  \\
%  Simple Greedy & 4 & 4 & 0 & N/A & N/A & 0.5762 & 0.6816   \\
%  Exhaustive & 20 & 0 & 4 & 0.5922 & \textbf{0.6989} & 0.5964 & 0.7049   \\
%  Exhaustive & 20 & 4 & 0 & \textbf{0.5925} & 0.6902 & 0.5964 & 0.6998   \\
%  Greedy & 41 & 0 & 4 & 0.5857 & 0.6972 & \textbf{0.5971} & 0.7084  \\
%  Greedy & 41 & 1 & 3 & 0.5767 & 0.6929 & 0.5863 & 0.\textbf{7097}    \\
%  Greedy & 41 & 2 & 2 & 0.5837 & 0.6932 & 0.5864 & 0.7089    \\
%  Greedy & 41 & 3 & 1 & 0.5883 & 0.6853 & 0.5857 & 0.7060    \\
%  Greedy & 41 & 4 & 0 & 0.5897 & 0.6922 & 0.5907 & 0.6981    
% \end{tabular}
% \caption{Comparison of Search Strategies.  All experiments run without normalization using the max aggregator.  We find that using the greedy approach optimizing all models for long answer F1 generalizes best to the ``dev-test'' set for short answer F1 and is only slightly lower than the best long answer F1.  The search and eval scores refer to ``dev-train'' and  ``dev-test'' respectively.}
% \label{tab:exp:ens:search}
% \end{table*}

% We first investigate the different search strategies in table \ref{tab:exp:search}.  We see that the simple greedy approach is not as good as either the exhaustive or greedy approaches\footnote{Note that the models were selected based on dev set performance rather than ``dev-train`` performance yielding optimistic eval scores, however they are still lower than for the other approaches.} and further note that the simple greedy ensemble optimized for long answers outperforms the one optimized for short answers on both short and long answers on the ``dev-test'' set.  For the exhaustive approach we see that it obtains the best long and short F1 scores on ``dev-train'' for the respective models as expected, however these do not translate to the best scores on ``dev-test''.  We find that the greedy approach performs best overall, with the greedy ensemble optimized exclusively for long answer performance performing the best on short answer F1 and is 0.0013 F1 lower than the best long answer F1 on ``dev-test''.  Also note that the numbers seen here, praticularly when optimizing greedily ofr long answer performance are higher than those observed for ensembling the same model with multiple seeds in table \ref{tab:exp:seed}.

% We hypothesize \anthony{TODO better word?} that the reasons for the superior generalization of the greedy approach over exhaustive is that exhaustive search is ``overfitting''.  Another potential cause of the better generalization of greedy is that it can search more candidates.  Whereas with the greedy approach we can search all 41 candidates\footnote{candidate models represent models trained with different model types (e.g. BERT for QA and AoA) and hyperparameters (e.g. learning rate and negative example subsampling rate)}, with exhaustive search we only consider our top 20 (by sum of short and long answer F1) for runtime considerations.  This gives the greedy strategy a more diverse set of candidates to work with.  Similarly we hypothesize the reason optimizing for long answer F1 generalizes better for short and long answers is due to the strict definition of correctness for Natural Questions which requires exact span matching \cite{Kwiatkowski2019NaturalQA}.  For the remainder of this paper we will focus on greedy search with all four models optimized for long answer to keep the number of experiments presented to a manageable level.  Note that further experimentation with different short and long answer optimization trade-offs confirm the conclusion here that optimizing for long answer performance generalizes the best.

% % - Greedy with all candidates vs candidates chosen from exhaustive [Num models searched, Num SA models, Num LA models, SA F1 Search, LA F1 Search, F1 F1 Eval, LA F1 Eval]
% %     - Conclusion: There is some benefit to using all candidates (and it’s quick enough with greedy) to use all

% \begin{table*}[]
% \small
% \begin{tabular}{lllll}
% \# Models Searched  & SA F1 Search & LA F1 Search & SA F1 Eval & LA F1 Eval   \\
% 41  & 0.5857 & \textbf{0.6972} & \textbf{0.5971} & \textbf{0.7084}  \\
% 20  & \textbf{0.5860} & 0.6951 & 0.5896 & 0.704    
% \end{tabular}
% \caption{Impact of candidate pool size.  All experiments run with a greedy search strategy optimized exlcusively for long answer F1 without normalization using the max aggregator.  We find that the using the entire candidate model pool produces an increase in both long and short answer F1.}
% \label{tab:exp:ens:candidates}
% \end{table*}

% In table \ref{tab:exp:ens:candidates} we investigate the impact of the candidate model search space size.  We use the greedy search strategy to optimize for long answer performance without normalization using the max aggregator.  For the experiment with 20 candidates we use the same 20 candidates as for the exhaustive search strategy experiment (greatest sum of short and long answer F1s).  We find that the added diversity of the models avaible in the entire pool produces a stronger ensemble which generalizes better both in short and long answer F1.  Having verified the benefit of using the entire candidate pool we continue to do so in the remainder of our experiments.


% % - Greedy Sum [Num SA models, Num LA models, SA F1 Search, LA F1 Search, F1 F1 Eval, LA F1 Eval]
% %     - Conclusion: sum is worse than max
% %     - Would like to do something better than make a table just for this but noting immediately comes to mind
% %     - I also have exhaustive sum if we think it would be good to add that
% %     - I’m assuming when we cut this will be one of the first tables to go

% \begin{table*}[]
% \small
% \begin{tabular}{lllll}
% Aggregation Strategy  & SA F1 Search & LA F1 Search & SA F1 Eval & LA F1 Eval   \\
% Max  & \textbf{0.5857} & \textbf{0.6972} & \textbf{0.5971} & \textbf{0.7084}  \\
% Sum  & 0.4382 & 0.6873 & TODO & TODO    
% \end{tabular}
% \caption{Comparison of max and sum aggregation strategies.  All experiments run with a greedy search strategy optimized exclusively for long answer F1 without normalization.  We find that the using the max aggregator results in better short and long answer F1.}
% \label{tab:exp:ens:sum}
% \end{table*}

% We compare the results of the sum and max aggregators in table \ref{tab:exp:ens:sum}.  All experiments are run with the greedy search strategy over the full pool of 41 candidates without normalization. \anthony{TODO: run eval numbers for sum and add results to table and here}


% % - Greedy Normalized with different aggregation types [Aggregation strategy, Num SA models, Num LA models, SA F1 Search, LA F1 Search, F1 F1 Eval, LA F1 Eval]
% %     - Conclusion: Noisy Or helps LA, all approaches hurt SA

% \begin{table*}[]
% \small
% \begin{tabular}{lllll}
% Aggregation Strategy  & SA F1 Search & LA F1 Search & SA F1 Eval & LA F1 Eval   \\
% Max  & \textbf{0.5857} & 0.6972 & \textbf{0.5971} & 0.7084  \\
% Exponential Sum  & 0.5619 & 0.6944 & 0.5826 & 0.7040  \\
% Linear Sum  & 0.5553 & 0.6954 & 0.5728 & 0.7066  \\
% Noisy Or  & 0.5545 & \textbf{0.7037} & 0.573 & \textbf{0.715}  
% \end{tabular}
% \caption{Comparison of IR inspired aggregation strategies.  All experiments run with a greedy search strategy optimized exclusively for long answer F1 with logistic regression normalization (except max which is not normalized).  We find that the using the noisy or aggregator improves long answer F1, however all strategies decrease short answer F1.}
% \label{tab:exp:ens:norm-agg}
% \end{table*}

% We investigate the impact of the IR inspired normalization strategies in table \ref{tab:exp:ens:norm-agg}.  The max experiment is as-before run without normalization to greedily optimize for long answer F1.  The other experiments here are normalization with logistic regression, as our experiments showed that not normalizing decreased performance.  We find that using max aggregation results in the best short answer F1 whereas using normalized noisy or aggregation results in the best long answer F1.


% % - I also have a couple follow up experiments which I would like to put in a table, but the descriptions of them would be a little much to put in a table
% %     - Conclusion: Use Noisy or (normalized) on LA and max (unnormalized) on SA.  Also, selecting candidates by using Greedy then doing noisy or for LA and max for SA may help both LA and SA performance (+~0.3-0.4 each F1 on ~3200 examples)

% \anthony{TODO: update below table with new expt numbers}

% \begin{table}[]
% \small
% \begin{tabular}{lll}
% Model Selection Aggregation Strategy  & SA F1 Eval & LA F1 Eval   \\
% Max  & \textbf{0.5971} & \textbf{0.7179} \\
% Noisy Or  & 0.5934 & 0.7150 \\
% \end{tabular}
% \caption{Experiments using unnormalized max for short answers and logistic regression normalized noisy or for long answers.  For these experiments the ensembled models are those selected from the max and noisy or experiments respectively in table \ref{tab:exp:ens:norm-agg}.  Using candidates selected with max allows ensembles to be found faster as logisitc does not need to be repeatedly run in the search phase.  We find that selecting models in this way does not decrease performance. \anthony{TODO: significance phrasing?}}
% \label{tab:exp:combine}
% \end{table}

% \anthony{TODO: Probably revise to clarify meaning of expt}


% We investigate the effectiveness of extending the approach from \ref{tab:exp:combine} by changing the core strategy so that short answers are required to be contained in the best long answer.  This follows from a requirement of \cite{Kwiatkowski2019NaturalQA} that short answers be contained in the long answer (if there is a short answer).  Surprisingly we find in table \ref{tab:exp:restrict-sa-to-la} that this decreases short answer performance.  We hypothesize that this is a result of incorrect long answer predictions forcing the system to predict an incorrect short answer, but leave a more formal examination to future work.

% \begin{table}[]
% \small
% \begin{tabular}{ll}
% Short Answer Containing Span  & SA F1 Eval    \\
% Any non-null  & \textbf{0.5971}  \\
% Best long span  & 0.5836  
% \end{tabular}
% \caption{Investigation of requiring short span predictions to be contained within the predicted long span.  We find that doing so decreases short answer performance.}
% \label{tab:exp:restrict-sa-to-la}
% \end{table}

% \anthony{TODO: update these numbers as well after running expts with no snoop normalizer.  Probably revise to clarify meaning of expt}

% Based on our conclusions from table \ref{tab:exp:ens:norm-agg} that unnormalized max works best for short answers and logistic regression normalized noisy or works best for long answers we experiment with this configuration in table \ref{tab:exp:combine}.  We find that this approach produces the strongest performance for both short and long answers.  Further, we investigate selecting models using unnormalized max for both short and long answers, and then running with logistic regression normalized noisy or on the ``dev-test'' set.  This allows for a quicker ensemble model selection as logisitc does not need to be repeatedly run in the search phase.  We find that this approach does not decrease short answer or long answer F1 performance \anthony{TODO: significance to claim increases???}.  In conclusion, we recommend using unnormalized max for short answers and logistic regression normalized noisy or for long answers when running an ensemble with models selected using unnormalized max for both short and long answer (for quicker model selection).
